BP-MPC: Optimizing the Closed-Loop Performance of MPC using BackPropagation

Model predictive control (MPC) is pervasive in research and industry. However, designing the cost function and the constraints of the MPC to maximize closed-loop performance remains an open problem. To achieve optimal tuning, we propose a backpropagation scheme that solves a policy optimization problem with nonlinear system dynamics and MPC policies. We enforce the system dynamics using linearization and allow the MPC problem to contain elements that depend on the current system state and on past MPC solutions. Moreover, we propose a simple extension that can deal with losses of feasibility. Our approach, unlike other methods in the literature, enjoys convergence guarantees.

==> Contents/0_title_and_authors.tex <==

\title{Iterative predictive control for uncertain systems satisfying quadratic inequalities}

\author{Riccardo Zuliani, Efe C. Balta, , John Lygeros
% \thanks{R. Zuliani, E. C. Balta, A. Rupenyan and J. Lygeros are with the Automatic Control Laboratory, ETH Zurich, 8092 Zurich, Switzerland. A. Rupenyan is also with Inspire AG, 8092 Zurich, Switzerland \texttt{\small$\{$rzuliani,ebalta,ralisa,lygeros$\}$@control.ee.ethz.ch}.}
}

% The paper headers
% \markboth{IEEE TRANSACTIONS ON MICROWAVE THEORY AND TECHNIQUES, VOL.~60, NO.~12, DECEMBER~2012
% }{Roberg \MakeLowercase{\textit{et al.}}: High-Efficiency Diode and Transistor Rectifiers}


\maketitle

==> Sources/header.tex <==
% Necessary definitions for template
\usepackage{generic}

\usepackage{textcomp}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%\markboth{\hskip25pc IEEE TRANSACTIONS AND JOURNALS TEMPLATE}
%{Zuliani \MakeLowercase{\textit{et al.}}: BP-MPC}

% References
\usepackage{cite}
\usepackage{csquotes}
\usepackage[english]{babel}

% Algorithms
\RequirePackage{algorithm,algpseudocode}
\algnewcommand\algorithmicinit{\textbf{Init:}}
\algnewcommand\Init{\item[\algorithmicinit]}
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

% tables
\usepackage{booktabs}
\usepackage{subcaption}
\DeclareCaptionFormat{custom}
{%
    \sffamily\footnotesize #1.\, #3
}
\captionsetup{format=custom}

% Math packages
\usepackage{amssymb,amsfonts,mathrsfs}
\usepackage{amsmath}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}

% Fonts
\usepackage{stmaryrd}
\usepackage[cal=cm,bb=ams]{mathalpha} % Improve calligraphic and bb math
\renewcommand{\ttfamily}{\fontencoding{T1}\fontfamily{lmtt}\selectfont}

% Additional math options
\usepackage{xspace}
\usepackage{derivative}

% Hyperlinks and referencing
\makeatletter
\let\NAT@parse\undefined
\makeatother
\PassOptionsToPackage{hyphens}{url}\usepackage[hidelinks]{hyperref}
\usepackage[nameinlink,sort]{cleveref}

% fix for references in titles
\makeatletter
\patchcmd{\@bibitem}{\ignorespaces}{\label{bib-#1}\ignorespaces}{}{}
\makeatother

% cite in titles
\newcommand{\mycite}[1]{[\ref{bib-#1}]}
\newcommand{\mytcite}[1]{\texorpdfstring{\cite{#1}}{\mycite{#1}}}

% Figures
% \usepackage[dvipsnames]{xcolor}
\usepackage{graphicx}

% Clever ref names
\crefname{appendix}{Appendix}{Appendices}
\AtBeginEnvironment{appendices}{\crefalias{section}{appendix}}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{theorem}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{section}{Section}{Sections}
\crefname{proposition}{Proposition}{Propositions}
\crefname{equation}{}{}
\crefmultiformat{equation}{(#2#1#3}{, #2#1#3)}{, #2#1#3}{, #2#1#3)}
\crefrangeformat{equation}{(#3#1#4-#5#2#6)}
\crefrangeformat{assumption}{Assumptions #3#1#4-#5#2#6}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{subsection}{Subsection}{Subsections}
\crefname{paragraph}{Paragraph}{Paragraph}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefname{remark}{Remark}{Remark}
\crefname{table}{Table}{Table}

% theorems
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

% commands for referencing problems
% \newcommand{\mpc}{\hyperlink{PF_mpc}{MPC$(\bar{p})$}\xspace}
\newcommand{\mpc}{$\mathrm{MPC}(\bar{p})$\xspace}
% \newcommand{\mpce}{\hyperlink{PF_mpc}{MPC$(\bar{x}_t,p)$}\xspace}
\newcommand{\mpce}{\ensuremath{\mathrm{MPC}(\bar{x}_t,p)}\xspace}
% \newcommand{\qp}{\hyperlink{eq:DIFF_QP}{QP$(\bar{p})$}\xspace}
\newcommand{\qp}{\eqref{eq:DIFF_qp}\xspace}
% \newcommand{\dual}{\hyperlink{eq:PF_dual}{D$(\bar{p})$}\xspace}
\newcommand{\dual}{\eqref{eq:DIFF_dual}\xspace}

% Math commands
\DeclareMathOperator*{\argmin}{arg\,min}

% Counter for double columns equations
\newcounter{MYtempeqncnt}

% Footnotes in tables
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

% Tikz
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usetikzlibrary{plotmarks}
\usetikzlibrary{shapes,arrows,decorations.markings}
\usetikzlibrary{arrows.meta}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{calligraphy}
\usepackage{tkz-euclide}
\usepackage{hf-tikz}
\usetikzlibrary{decorations.pathreplacing}
\usepgfplotslibrary{groupplots}
% Tikz custom blocks
\usetikzlibrary{plotmarks}

% add external pdfs
\usepackage{pdfpages}
